Fathom-Vaidya: Advancing Medical Reasoning with Rubric-Based Rewards

Deploying Large Language Models (LLMs) in healthcare requires robust performance across two complementary dimensions - diagnostic reasoning: the convergent, evidence-driven task of inferring a patient's condition from clinical data to produce a diagnosis, and clinical healthcare reasoning: the broader, navigational judgment required to communicate, plan, and adapt across multi-turn clinical interactions where a single correct answer may not exist. Recent benchmarks such as HealthBench and MedXpertQA reveal persistent weaknesses in both areas, exposing failures in complex diagnostic scenarios and limitations in contextual, patient-centered dialogue. We introduce a sequential training framework that targets these facets using synthetic data and rubric-based reinforcement learning. First, we improve diagnostic reasoning using MedBullets-derived questions with rule- and rubric-guided Reinforcement Learning (RL). We then shift to clinical reasoning by generating 5.3k synthetic multi-turn scenarios, each paired with multi-dimensional rubrics to comprehensively assess the response. This approach yields over 10% improvement on MedXpertQA, and our 30B model achieves 50.1% accuracy on HealthBench-Hard, surpassing proprietary baselines including GPT-5 (thinking). Our results show that targeted synthetic datasets and rubric-based training can systematically improve both diagnostic and interactive clinical reasoning in medical LLMs.

==> tex_files/tables/ablation.tex <==
\begin{table}[ht]
% \setlength{\abovecaptionskip}{0.3cm}
% \setlength{\belowcaptionskip}{-0.1cm}
\centering
\caption{Accuracy scores (\%) over healthbench-hard (with system prompt) while training on \synhb and healthbench-easy}
%\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c}
\hline
\textbf{Model} & \textbf{Score} \\
\hline
Qwen3-4B-Ablation & 34.03 \\
FV-4B & 35.30 (+1.27\%) \\
\hdashline
Qwen3-8B-Ablation & 28.20 \\
FV-8B & 40.15 (+11.95\%) \\
\hdashline
Qwen3-30B-A3B-Ablation & 36.55 \\
FV-30B-A3B & 49.35 (+12.80\%)\\
\hline
\end{tabular}
%}
\label{tab:ablation}
\end{table}

==> tex_files/tables/qs_distribution_medb.tex <==
\begin{table}[ht]
% \setlength{\abovecaptionskip}{0.3cm}
% \setlength{\belowcaptionskip}{-0.1cm}
%\centering
\caption{Distribution of questions across topics in Medbullets}
% \resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|c}
\hline
Broad Topic & $\%$ of Questions \\%%& \textbf{VAIDYA} \\
\hline
Foundational Basic Sciences & 35$\%$\\
Organ System-Based Medicine & 30$\%$\\
Pathology \& Disease Mechanisms & 20$\%$\\
Reproductive Medicine & 7$\%$\\
Psychiatry \& Behavioral Science & 5$\%$\\
General Topics & 3$\%$\\

\hline
\end{tabular}
% }
\label{tab:qs_dist_medb}
\end{table}

==> tex_files/tables/theme_distribution.tex <==
\begin{table}[ht]
% \setlength{\abovecaptionskip}{0.3cm}
% \setlength{\belowcaptionskip}{-0.1cm}
%\centering
\caption{Distribution of cases across themes in \synhb}
% \resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|c}
\hline
Theme & Count ($\%$) \\%%& \textbf{VAIDYA} \\
\hline
Responding under uncertainty & 1024 (19.14$\%$)\\
Global health & 965 (18.03$\%$)\\
Expertise-tailored communication & 679 (12.69$\%$)\\
Emergency referrals & 497 (9.29$\%$)\\
Health data tasks & 350 (6.54$\%$) \\
Context seeking & 225 (4.2$\%$)\\

\hline
\end{tabular}
% }
\label{tab:theme_dist}
\end{table}
